RealDiffFusionNet: Neural Controlled Differential Equation Informed Multi-Head Attention Fusion Networks for Disease Progression Modeling Using Real-World Data

This paper presents a novel deep learning-based approach named RealDiffFusionNet incorporating Neural Controlled Differential Equations (Neural CDE) - time series models that are robust in handling irregularly sampled data - and multi-head attention to align relevant multimodal context (image data, time invariant data, etc.) at each time point. Long short-term memory (LSTM) models were also used as a baseline. Two different datasets were used: a data from the Open-Source Imaging Consortium (OSIC) containing structured time series data of demographics and lung function with a baseline CT scan of the lungs and the second from the Alzheimer's Disease Neuroimaging Initiative (ADNI) containing a series of MRI scans along with demographics, physical examinations, and cognitive assessment data. An ablation study was performed to understand the role of CDEs, multimodal data, attention fusion, and interpolation strategies on model performance. When the baseline models were evaluated, the use of multimodal data resulted in an improvement in Neural CDE performance, with a lower test RMSE. Additionally, the performance of multimodal Neural CDE was also superior to multimodal LSTM. In the attention-based architectures, fusion through concatenation and rectilinear interpolation were found to improve model performance. The performance of the proposed RealDiffFusionNet was found to be superior (0.2570) to all models. For the ADNI dataset, between the Neural-CDE and LSTM models trained only on the structured data, the test RMSE were comparable (0.471 for LSTM vs. 0.4581 Neural-CDE). Furthermore, the addition of image features from patients' MRI series resulted in an improvement in performance, with a lower test RMSE (0.4372 with multimodal vs 0.4581 with structured data). RealDiffFusionNet has shown promise in utilizing CDEs and multimodal data to accurately predict disease progression.

==> subfiles/experiments.tex <==
\section{Results and Discussion}
\subsection{Structured Data}
Figure~\ref{fig:struct_plots} reveals a compelling pattern with structured data alone. 
When contrasting the model predictions and actual values, we find that they align closely with the line of unity, indicating the model performed well. 
Yet, upon closer inspection, we observe that the predictions offered by the Neural-CDE models display less variation from this line. 
This shows a stronger correlation between the actual values and the predicted values, pointing to superior performance from the Neural-CDE models relative to the LSTM models.

Moreover, by examining plots representing the disease progression of a selected patient, we can deduce that both models have successfully captured the general trends of disease progression. 
This capability showcases the models' predictive power in reflecting the dynamic nature of patient health over time. 

% Insert a figure:
\begin{figure}[ht] %h means here, t means top, and b means bottom
    \centering
    \includegraphics[width=0.45\textwidth]{Picture5.png}
    \caption{Actual vs. Predicted FVC values and Pulmonary Fibrosis Progression with Structured Data}
    \label{fig:struct_plots}
\end{figure}

Table~\ref{tab:structured_metrics} provides a comprehensive comparison of the performance of the LSTM and Neural-CDE models when applied to structured data. The table clearly shows the superior performance of the Neural CDE models across both datasets when tested.

\begin{table}[!htp]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models & \multicolumn{9}{c}{Metrics} \\
\cmidrule(l){2-10}
& \multicolumn{3}{c}{RMSE} & \multicolumn{3}{c}{$R^{2}$}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(l){8-10}
& {Train} & {Validation} & {Test} & {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.2224 & 0.2381 & 0.3745 & 0.6610 & 0.1980 & 0.8515 \\
Neural CDE & 0.2789 &  0.3256 & \B 0.2693 & 0.8922 & 0.7464 & \B 0.9149 \\
\bottomrule
\end{tabular}

\caption{Model Evaluation Metrics for Structured Data}
\label{tab:structured_metrics}
\end{table}

Using structured data alone, Root Mean Square Error ($RMSE$) observed with the Neural CDE model was 0.2693, which is lower than the LSTM model's RMSE of 0.3745. 
A lower RMSE indicates a model's predictions are, on average, closer to the actual values, signifying higher precision. 
Furthermore, the Neural CDE model achieved a coefficient of determination, or $R^{2}$ score, of 0.9149, which surpasses the LSTM's score of 0.8515. 
A higher $R^{2}$ score signifies that the model explains a greater proportion of the variance in the dependent variable, denoting a higher level of accuracy.

\subsection{Multimodal Data}

When the predictions of both the LSTM and Neural-CDE models trained on multimodal data were compared, as seen in Figure\ref{fig:multi_plots}, an improvement has been realized over models that utilize only structured data. 
This enhancement can be attributed to the contextual information provided by the CT image data, which augments the predictive power of both LSTM and Neural-CDE models. 
Furthermore, there is a discernible decrease in the deviation of the predicted versus the actual observed values from the line of unity. 
This suggests an increased alignment of the predicted outcomes with the actual data, denoting a higher level of precision and accuracy in the model predictions when multimodal data is employed. 
Furthermore, it was observed that the multimodal Neural-CDE model achieved super performance in alignment with predicted outcomes versus the actual data. 
Additionally, the disease progression curves from the LSTM and Neural-CDE models trained on multimodal data closely mirror each other, indicating a robust overlap. 

% Insert a figure:
\begin{figure}[h] %h means here, t means top, and b means bottom
    \centering
    \includegraphics[width=0.45\textwidth]{Picture6.png}
    \caption{Actual vs. Predicted FVC values and Pulmonary Fibrosis Progression with Multimodal Data}
    \label{fig:multi_plots}
\end{figure}

\begin{table}[!htp]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models & \multicolumn{9}{c}{Metrics} \\
\cmidrule(l){2-10}
& \multicolumn{3}{c}{$RMSE$} & \multicolumn{3}{c}{$R^{2}$}  \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(l){8-10}
& {Train} & {Validation} & {Test} & {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.1962 & 0.3491 & 0.3321 & 0.3400 & 0.5109 & 0.8742 \\
Neural CDE & 0.2789 &  0.3256 & \B 0.2693 & 0.0712 & 0.548 & \B 0.9368 \\
\bottomrule
\end{tabular}

\caption{Model Evaluation Metrics for Multimodal Data}
\label{tab:multi_metrics}
\end{table}

Based on model evaluation metrics (Table 2) the Neural-CDE model outperforms the LSTM model using multimodal data. It achieves an RMSE of 0.2353, which is lower than the LSTM's RMSE of 0.3321, demonstrating its superior precision in this context as well. Furthermore, the Neural-CDE model recorded an R2 score of 0.9368, higher than the LSTM's R2 score of 0.8742, pointing to its higher accuracy in predicting the disease progression. 

These findings reinforce the notion that the Neural CDE model demonstrates a higher predictive power when compared to the LSTM model, especially when applied to the OSIC dataset. By all indications, it exhibits more precise and accurate predictions, making it the more reliable choice for tasks involving both structured and multimodal data.

Our analysis indicates a notable trend across both the Neural-CDE and LSTM models: those that integrated multimodal data, including the patient’s baseline CT scan, exhibited superior performance in the test set.

Looking first at the Neural-CDE model using structured data, we observed an RMSE of 0.2693 and an $R^{2}$ score of 0.9149. 
However, when we transitioned to using multimodal data, the performance metrics improved, with the RMSE dropping to 0.2353 and the $R^{2}$ score rising to 0.9368. 
This demonstrates an increase in both the precision and accuracy of the model when enriched with the multimodal data.

Similarly, the LSTM model displayed enhanced performance when using multimodal data. 
When solely structured data was utilized, the RMSE stood at 0.3745 and the $R^{2}$ score was 0.8515. 
However, the model that incorporated multimodal data showed a reduced RMSE of 0.3321 and an increased $R^{2}$ score of 0.8742. 
The improvement seen in both these models underscores the value of including image modality data in our analysis, which allows the model to capture more nuanced information.

Furthermore, Hamdi et al. \cite{hamdi2021marl} evaluated numerous machine learning algorithms using the OSIC dataset and put forward a state-of-the-art Multimodal Attention Model using LSTM and EfficientNet (MARL) that achieved an R2 of 91\%. 
Notably, our proposed multimodal Neural-CDE model outperformed this, attaining an R2 of 94\%. 
The superior performance of our model is believed to stem from the incorporation of the Neural-CDE, which has shown to handle irregularly sampled data effectively. 
This characteristic is instrumental in boosting the model's performance with the OSIC dataset, making it a strong contender for future predictive tasks in similar scenarios.

\subsection{LSTM vs Neural CDE Multifusion}

\begin{table}[!htp]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models %& \multicolumn{9}{c}{$RMSE$} \\
\\ %\multicolumn{3}{c}{$R^{2}$}  \\
%\cmidrule(lr){2-4} \cmidrule(lr){5-7} \\ %\cmidrule(l){8-10}
& {Train} & {Validation} & {Test} \\ %& {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.3038 &  0.8191 &  0.9066 \\ %& 0.0712 & 0.548 & \B 0.9368 \\
Neural CDE & 0.0859 & 0.3854 & \B 0.2912 \\ %& 0.3400 & 0.5109 & 0.8742 \\ 
\bottomrule
\end{tabular}

\caption{Interpolation Schemes}
\label{tab:interpolation_metrics}
\end{table}

\begin{table}[!htp]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models %& \multicolumn{9}{c}{$RMSE$} \\
\\ %\multicolumn{3}{c}{$R^{2}$}  \\
%\cmidrule(lr){2-4} \cmidrule(lr){5-7} \\ %\cmidrule(l){8-10}
& {Train} & {Validation} & {Test} \\ %& {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.3038 &  0.8191 &  0.9066 \\ %& 0.0712 & 0.548 & \B 0.9368 \\
Neural CDE & 0.0859 & 0.3854 & \B 0.2912 \\ %& 0.3400 & 0.5109 & 0.8742 \\ 
\bottomrule
\end{tabular}

\caption{Comparing Interpolation Schemes}
\label{tab:interpolation_metrics}
\end{table}

\subsection{LSTM vs Neural CDE Multifusion}

\begin{table}[!htp]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models %& \multicolumn{9}{c}{$RMSE$} \\
\\ %\multicolumn{3}{c}{$R^{2}$}  \\
%\cmidrule(lr){2-4} \cmidrule(lr){5-7} \\ %\cmidrule(l){8-10}
& {Train} & {Validation} & {Test} \\ %& {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.3038 &  0.8191 &  0.9066 \\ %& 0.0712 & 0.548 & \B 0.9368 \\
Neural CDE & 0.08594 & 0.3854 & \B 0.2912 \\ %& 0.3400 & 0.5109 & 0.8742 \\ 
\bottomrule
\end{tabular}

\caption{LSTM vs Neural CDE Multifusion}
\label{tab:multifusion_metrics}
\end{table}

\subsection{Attention Fusion Mechanisms}

\begin{table}[!h]
\centering

\sisetup{detect-all}
\NewDocumentCommand{\B}{}{\fontseries{b}\selectfont}

\begin{tabular}{
  @{}
  l
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=-1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  S[table-format=1.2]
  @{}
}
\toprule
Models %& \multicolumn{9}{c}{$RMSE$} \\
\\ %\multicolumn{3}{c}{$R^{2}$}  \\
%\cmidrule(lr){2-4} \cmidrule(lr){5-7} \\ %\cmidrule(l){8-10}
& {Train} & {Validation} & {Test} \\ %& {Train} & {Validation} & {Test}  \\
\midrule
LSTM & 0.3038 &  0.8191 &  0.9066 \\ %& 0.0712 & 0.548 & \B 0.9368 \\
Neural CDE & 0.0859 & 0.3854 & \B 0.2912 \\ %& 0.3400 & 0.5109 & 0.8742 \\ 
\bottomrule
\end{tabular}

\caption{Comparing Attention Fusion Mechanisms}
\label{tab:fusion_metrics}
\end{table}
